Explorable Parity Automata

We define the class of explorable automata on finite or infinite words. This is a generalization of History-Deterministic (HD) automata, where this time non-deterministic choices can be resolved by building finitely many simultaneous runs instead of just one. We show that recognizing HD parity automata of fixed index among explorable ones is in PTime, thereby giving a strong link between the two notions. We then show that recognizing explorable automata is ExpTime-complete, in the case of finite words or parity automata up to index [0, 2]. Additionally, we define the notion of Ï‰-explorable automata on infinite words, where countably many runs can be used to resolve the non-deterministic choices. We show ExpTime-completeness for Ï‰-explorability of automata on infinite words for the safety and coBÃ¼chi acceptance conditions. We finally characterize the expressivity of (Ï‰-)explorable automata with respect to the parity index hierarchy.

==> macros.tex <==
 \usepackage[utf8]{inputenc}
% \usepackage[a4paper, margin=2cm]{geometry}
 

%to avoid font warnings
\RequirePackage{silence}
\WarningFilter{latexfont}{Font shape}

%for pictures
\graphicspath{{figures/}}

\usepackage{proof}
%\usepackage{ebproofs}
\usepackage{amsmath}
%\usepackage{cleveref}
%\usepackage{todonotes}
%\usepackage{anyfontsize}
\usepackage{amsthm}
\usepackage{tabu}
\usepackage{textcomp}
%\usepackage{enumitem}
\usepackage{amssymb}
\usepackage{stmaryrd}
\usepackage{dsfont}
\usepackage{pgf}
\usepackage{tikz}
\usepackage{wasysym}
\usepackage{xspace}
\usetikzlibrary{arrows,automata, positioning, calc}
\usepackage{comment}
\usepackage{float}
\usepackage{todonotes}

\usepackage[hidelinks,breaklinks]{hyperref}

\usepackage{cleveref}


\crefname{exa}{Example}{Examples} % For cref
\crefname{defi}{Definition}{Definitions} % For cref
\crefname{thm}{Theorem}{Theorems}
\crefname{thmC}{Theorem}{Theorems}
\crefname{lem}{Lemma}{Lemmas}
\crefname{cor}{Corollary}{Corollaries}
\crefname{rem}{Remark}{Remarks}


\usepackage{ifthen}
\newboolean{shortver}
\setboolean{shortver}{false}% for short version 
%if short version, make sure applabels is up-to-date to correctly refer to the appendix. It is produced by taking the relevant newlabels in the .aux
%\setboolean{shortver}{false}% for long version


%switch between long and short version, with
% \ifthenelse{\boolean{shortver}}{% 
%    %short version content
%    }{% 
%    %long version content
%    }

\newcommand{\shortlong}[2]{\ifthenelse{\boolean{shortver}}{#1}{#2}}
%usage \shortlong{short_ver}{long_ver}
\newcommand{\app}[1]{\shortlong{the long version (Appendix #1)}{Appendix #1}}

%to reference the appendix and include its citations in short version.
%applabels.tex is obtained by taking the relevant \newlabel{..} in the .aux file
\shortlong{\input{applabels}}{}
%usage : \app{\ref{refname}}

\newcommand{\denis}[1]{\textcolor{red}{#1}}
\newcommand{\emile}[1]{\textcolor{blue}{#1}}
\def\bra#1{\langle#1\rangle}
\def\o{\textopenbullet\space}
\def\b{\textbullet\space}
\def\Acc{\mathit{Acc}}
\def\A{\mathcal{A}}
\def\B{\mathcal{B}}
\def\C{\mathcal{C}}
\def\D{\mathcal{D}}
\def\E{\mathcal{E}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\I{\mathcal{I}}
\def\K{\mathcal{K}}
\def\L{\mathcal{L}}
\def\M{\mathcal{M}}
\def\P{\mathcal{P}}
\def\Q{\mathcal{Q}}
\def\R{\mathcal{R}}
\def\T{\mathcal{T}}
\def\r#1{\textcolor{red}{#1}}
\def\g#1{\textcolor{teal}{#1}}
\newcommand{\bracket}[1]{[#1]}

%theorem sans numero
\newtheorem*{theorem*}{Theorem}

%complexity
\newcommand{\PTIME}{\textsc{PTime}\xspace}
\newcommand{\EXPTIME}{\textsc{ExpTime}\xspace}
\newcommand{\PSPACE}{\textsc{PSpace}\xspace}
\newcommand{\EXPSPACE}{\textsc{ExpSpace}\xspace}

% Names of the players
\def\controller{Spoiler\xspace}
\def\agents{Determiniser\xspace}
\def\protector{Protector\xspace}
\def\eliminator{Eliminator\xspace}

% Blocks in omega hardness proofsketch
\def\configblock{Config\xspace}
\def\choicesblock{Choices\xspace}

\def\Eve{\exists}
\def\Adam{\forall}
\def\Evestate{E}
\def\Adamstate{A}
\newcommand{\Pos}{\textit{Pos}}
\newcommand{\Mem}{\textit{Mem}}
\newcommand{\Trans}{\textit{Trans}}
\def\Buchi{B\"uchi\;}
\def\omy{$\omega$-explorability\;}
\def\om{$\omega$-explorable\;}

\def\width{width\xspace}

\def\safe{\top}
\def\jail{\bot}
\def\store{\texttt{store}\xspace}
\def\qaM{q_f^\M}

\def\dom{\textrm{Dom}}
\def\im{\textrm{Im}}

\def\QA{Q}

\def\labelarrow#1{\overset{#1}{\longrightarrow}}
\def\trans#1{\labelarrow{#1}}
\def\atest{a_\mathrm{test}}

\def\sep{\texttt{Sep}}


\def\targ{f} %target state in population control
\def\Nbb{\mathbb{N}}
\def\N{\mathbb{N}}
\def\rk{\mathrm{rk}}

\def\blank{\textrm{\textvisiblespace}}


% Latin abreviations

\def\ie{\textit{i.e.}\xspace}
\def\eg{\textit{e.g.}\xspace}
\def\etc{\textit{etc.}\xspace}

\newcommand{\oi}[1]{\todo[color=green!40,caption={},size=\tiny]{#1}}
\newcommand{\oii}[1]{\todo[color=green!30,inline]{#1}}

\newcommand{\dk}[1]{\todo[color=blue!30,caption={},size=\tiny]{#1}}
\newcommand{\dki}[1]{\todo[color=blue!30,inline]{#1}}

% \newtheoremstyle{truc}
%   {3mm}% measure of space to leave above the theorem. E.g.: 3pt
%   {3mm}% measure of space to leave below the theorem. E.g.: 3pt
%   {}% name of font to use in the body of the theorem
%   {0pt}% measure of space to indent
%   {\bfseries}% name of head font
%   {:\newline}% punctuation between head and body
%   {0mm}% space after theorem head
%   {}% Manually specify head

% \theoremstyle{truc}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem*{definition}{Definition}
% \newtheorem*{conjecture}{Conjecture}
% \newtheorem*{example}{Example}
% \newtheorem*{remark}{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


